Towards a general model for psychopathology

The DSM-1 was published in 1952, contains 128 diagnostic categories, described in 132 pages. The DSM-5 appeared in 2013, contains 541 diagnostic categories, described in 947 pages. The field of psychology is characterised by a steady proliferation of diagnostic models and subcategories, that seems to be inspired by the principle of "divide and inflate". This approach is in contrast with experimental evidence, which suggests on one hand that traumas of various kind are often present in the anamnesis of patients and, on the other, that the gene variants implicated are shared across a wide range of diagnoses. In this work I propose a holistic approach, built with tools borrowed from the field of Artificial Intelligence. My model is based on two pillars. The first one is trauma, which represents the attack to the mind, is psychological in nature and has its origin in the environment. The second pillar is dissociation, which represents the mind defence in both physiological and pathological conditions, and incorporates all other defence mechanisms. Damages to dissociation can be considered as another category of attacks, that are neurobiological in nature and can be of genetic or environmental origin. They include, among other factors, synaptic over-pruning, abuse of drugs and inflammation. These factors concur to weaken the defence, represented by the neural networks that implement the dissociation mechanism in the brain. The model is subsequently used to interpret five mental conditions: PTSD, complex PTSD, dissociative identity disorder, schizophrenia and bipolar disorder. Ideally, this is a first step towards building a model that aims to explain a wider range of psychopathological affections with a single theoretical framework. The last part is dedicated to sketching a new psychotherapy for psychological trauma.

==> 07persdisord.tex <==
\section{Personality disorders}  
\label{sec:persdisord}

\subsection{Borderline Personality Disorder}

\subsubsection*{Introduction}

% BPD features 
\textbf{Borderline personality disorder (BPD)} \citep{gunderson2005} is characterized by a pervasive instability of mood, of personal relationships, of the perception of the self, identity and behavior. The central defense mechanism used by persons with BPD is splitting, which can be defined as the inability to integrate positive and negative aspects of the self and others. The result is a characteristic view of the world in ``black and white'' \citep{perry2013}. Another typical defense mechanism employed in BPD is projective identification, by which split-off parts of the self are projected into the object to exert possess and control \citep{klein1946}. As a result of using such defenses, persons with BPD often engage in idealization and devaluation of others, alternating between high positive regard and heavy disappointment.

% psychodynamic vision
The currently prevailing psychodynamic vision \citep{ahles2004} characterizes mental diseases (including BPD and NPD) based on the repertoire of associated defense mechanisms. Such defenses would be erected to overcome intrapsychic conflicts and/or wounds originating in the interaction between the future patient and the caregiver. According to O. Kernberg BPD and NPD share a so-called ``borderline personality organization'' \citep{kernberg1967}, conceptualized in terms of unintegrated and undifferentiated affects and representations of the self and others.

% common features: dissociation
In both BPD and NPD the unstable sense of self can lead to episodes of dissociation and chronic feelings of emptiness. Dissociation can take the form of depersonalization (feeling of separation from oneself and one's body), derealization (feeling of being detached from the external world), selective amnesia and emotional detachment \citep{radovic2002depers}.

\subsubsection*{Interpretation}

\begin{figure}[t] \begin{center} \hspace*{-0.00cm}
{\fboxrule=0.0mm\fboxsep=0mm\fbox{\includegraphics[width=17.00cm]{Picdir2/f01bubbles.png}}}
\caption{BPD: context map and emotional functioning. Some key contexts, such as ``mother relation'' and ``sexual relation'', are traumatic. In these contexts the functioning of the relational module is impaired: poles B and C are difficult to access in a non-dissociated condition, and the mind oscillates between poles A and D.}
\label{switchb}
\end{center} \end{figure}

%\colorbox{colhd}{behavioral scheme} \\
BDP is a complex condition, in which genetic and environmental factors are hypothesized to play a role. Childhood traumas involving caregivers are often present in the history of persons with BPD \citep{macintosh2015, elices2015}. As a result, the functioning of the relational module may be impaired in key contexts such as ``mother relation'' and ``sexual relation'' (Fig.~\ref{switchb}). In such contexts poles B and C are difficult to access, and the mind is forced to oscillate between poles A and D. When the mind falls into poles B or C, emotional dissociation is used to avoid re-living the painful emotions associated to the trauma.

%\colorbox{colhd}{BPD and emotions} \\
Despite the evident drawbacks of this behavior, the BPD person manages to keep his/her emotions while oscillating between the two sides of splitting, and only occasionally resorts to emotional dissociation, as a last defense line. The maintenance of the emotional part allows the BPD person to spend most of the time on a relatively high level of functioning. The BPD person is not happy when he/she experiences emotional detachment, he/she understands that something is wrong.

%\colorbox{colhd}{salience} \\
In the transition zone, the distortion and amplification of the features involved in traumatic situations has the purpose to warn the mind that it is nearing a traumatic pole. This is reminiscent of the phenomenon of ``aberrant salience'' which, according to some theories \citep{kapur2003salience}, is deemed responsible for the positive symptoms of schizophrenia (hallucinations and delusions). The salience mechanism would be mediated by the neurotransmitter dopamine: this would explain why antipsychotic drugs, that act by blocking the dopamine receptor, are effective in eliminating hallucinations. In contrast to the ``pure'' dopamine hypothesis of schizophrenia \citep{baumeister2002}, these theories explain why antipsychotic drugs have effect only after a period of time after the start of their administration. 

%\colorbox{colhd}{salience /2} \\
An intriguing possibility suggested by our model is that the phenomenon of aberrant salience in schizophrenia and the mechanism of feature distortion in the transition zone of a traumatic context could both be expressions of a standard warning mechanism used by the mind to stay away from traumatic poles. Transitory perceptual distortions or ``pseudo-hallucinations'' are present also in personality disorders \citep{gras2014}. The difference between such distortions and schizophrenic hallucinations would be quantitative rather than qualitative. The higher degree of severity of the hallucinatory symptoms in schizophrenia could be determined by a heavier traumatic charge and possibly mediated by a genetic predisposition. Another clinical example that could be explained by the phenomenon of feature distortion is the dysmorphic body image associated to eating disorders (among many other disorders) \citep{ruffolo2006}. 

\subsection{Narcissistic Personality Disorder}

\subsubsection*{Introduction}

% NPD features
The main characteristics of \textbf{narcissistic personality disorder (NPD)} \citep{lowen2004} are an excessive reference to others for self-esteem regulation, a deficit in the ability to feel empathy towards other individuals, a particular self-perception of the subject defined ``grandiose Self'', and a difficulty of emotional involvement. The exaggerated dependence on others for approval causes self-appraisal to oscillate between extremes. The person is characterized by a form of deep selfishness of which he/she is usually not aware. The consequences are likely to produce suffering, social problems or significant emotional and relational difficulties. NPD shares with BPD the use of splitting and projective identification as core defense mechanisms. 

\subsubsection*{Interpretation}

%\colorbox{colhd}{memory, emotional dissociation} \\
As in the case of BDP, it is not unreasonable to think that, besides genetic predisposing factors, childhood traumas may play a role in the development of NPD \citep{lowen2004}. As a result, the functioning of the relational module may be impaired in key contexts such as ``mother relation'' and ``sexual relation'' (Fig.~\ref{switchn}). In such contexts poles B and C cannot be accessed without dissociation and the mind is forced to oscillate between poles A and D. When the mind falls into poles B or C, emotional dissociation is used to avoid feeling the painful traumatic emotions.

%\colorbox{colhd}{NPD split} \\
Our assumption is that, in the NPD case, the traumas affecting a traumatic context are more severe. As a result, the forbidden and transition zones are more extended, so that the free zone around pole A is almost non-existent, while the free zone around pole D may still be present. Splitting is employed also by the NPD person, but with a different connotation. Pole D, in which a positive self unleashes its anger towards a frustrating and guilty object, is present also in NPD: the difference lies in pole A. While in the BPD case pole A is characterized by love and affection, in the NPD case love and affection do not belong to the repertoire of memories of the person, and therefore cannot be used to build a behavioral scheme for pole A. Instead of a scheme based on real life examples, the NPD person resorts to a fantasy: the bright side of his/her splitted reality is played by the grandiose self.

%\colorbox{colhd}{grandiose self} \\
The grandiose image is not associated to strong positive emotions: rather, it is imbued with a sense of victory and revenge for the past frustrations. Since pole A of NPD is not grounded on concrete experiences, is not associated to strong feelings and overall lays on very shaky grounds (such as the reward coming from the external world), it is much more volatile and unstable compared to pole A of BPD. When the world does not show enough empathy and/or provide sufficient reward, the NPD person jumps into pole D or is forced back into emotional dissociation. This is the state in which the NPD person spends most of his/her time. 

%\colorbox{colhd}{NPD dissociation} \\
This condition, characterized by emotional numbness, is not so disturbing for the NPD person as it is for the BPD person. This because the BPD person lives for most of the time in the world of emotions, and immediately perceives when dissociation kicks-in. The NPD person, on the contrary, is used to living without emotions: this is his/her normal condition. From the viewpoint of the emotional content, switching from the grandiose self to dissociation does not make much of a difference.    

%\colorbox{colhd}{psychopathy} \\
A reduced capacity to feel (certain) emotions is considered a central feature of antisocial personality disorder (APD) and psychopathy \citep{stevens2001facial, hastings2008}. This trait can be interpreted with our model if we assume that, in case of psychopaths, the negative poles B and C are not associated to strong emotional responses and therefore cannot be traumatized. Or, for this category of people, the capacity to dissociate would be so deep and pervasive as to eliminate the need for a transition zone in the feature space. If this were true, APD and psychopathy could be inserted into our framework as extreme cases of NPD. 

\newpage \mbox{}
\clearpage \pagebreak[4]


==> 08othercond.tex <==
\section{Other conditions: chronic pain, eating disorders}  
\label{sec:othercond}

\subsection{Chronic pain}

\subsubsection*{Introduction}

%\colorbox{colhd}{definitions and generalities} \\
The term chronic pain refers to a painful sensation that lasts a long time \citep{thienhaus2002}. Chronic pain may also be defined as a pain which loses its original function as a warning signal for a physical injury, and becomes an independent clinical entity on its own. Chronic pain can affect any region of the body, and display a variety of forms. Overall, it represents an important medical problem in society, with heavy psychological burden and high financial cost.

%\colorbox{colhd}{hysteric conversion} \\
The role played by the mind-body mutual interaction in the subjective experience of pain has been acknowledged for a long time. In conversion disorder (hysteria), a psychic conflict is unconsciously converted into symptoms with characteristics similar to those of a neurological disease \citep{akagi2001}. Symptoms include impaired coordination and balance, localised paralysis, loss of voice, pain, blindness, deafness, hallucinations, seizures. The onset is acute or subacute, and is linked to an event with strong emotional intensity and a clear symbolic reference. There are predisposing factors (mistreatment, abuse) and precipitating factors (stress, conflicts, losses).

%\colorbox{colhd}{Neuropathic pain} \\
Neuropathic pain is a chronic pain caused by the fact that, for a number of reasons, nerve fibers transmit wrong signals to pain centers located in the brain \citep{torrance2006}. This dysfunction of neurological activity may cause painful sensations even in the absence of real harm, or may affect the areas next to the injured ones, which become highly sensitive to pain. In this case, pain is not the symptom of a damage to a body part: it is the system of pain perception which is affected by an often irreversible damage. The ``bell'' is locked in the ``on'' position, and little can be done to stop it.

%\colorbox{colhd}{variability in pain response} \\
The perception of pain varies greatly among individuals \citep{gorczyca2013, mcgrath1994}. An example is given by low back pain, a very common problem at all latitudes. One of the physical conditions associated to back pain, vertebral disc degeneration, can be assessed through imaging techniques. However, the radiological situation does not always correlate with the subjective pain experience. In other words, there are individuals with persistent pain and a relatively good radiological situation, and individuals who have a worse radiological scenario and are pain-free. \citep{chou2006}.

%\colorbox{colhd}{emotional attitude} \\
The emotional attitude bears a high prognostic value for the evolution of pain. Pain tends to improve over time in individuals who do not pay much attention to it. On the contrary, in individuals with the tendency to ``catastrophising'' (i.e., ``I will suffer from pain for the rest of life'', ``I will be a disabled person'', etc.) episodic pain has a much greater chance to become chronic \citep{gorczyca2013, ong2015}.

\subsubsection*{Interpretation}

%\colorbox{colhd}{distortion} \\
In the transition zone ``defects'' (i.e. features which depart from prototypical values) appear distorted and magnified. The distortion of defects serves the purpose to warn the mind that the current situation is not prototypical anymore and it is drifting towards a bad pole. For instance, if ``making mistakes while playing the violin'' is a feature that carries a low level of worthiness (and thus contributes to lower the worthiness of the self), the slightest mistake appears magnified, distorted and threatening to the individual. The same mistake would appear much less threatening if the mind were in a different region of the feature space, away from the transition zone.

%\colorbox{colhd}{distorted pain} \\
Pain is also considered an unworthy feature by most people. The idea of pain is linked to lack of efficiency, to weakness, disability, etc, and all these features have very low worthiness values. Therefore, we should expect that the perception of pain be distorted and magnified in proximity of a bad pole. Interestingly, people with BPD often complain of persistent pain of various kinds \citep{sansone2012}. 

%\colorbox{colhd}{underlying features} \\
Based on this analysis, we can make some suggestions for a possible therapeutic intervention. The worthiness of the self and of the object depend all features associated to them. If the value of worthiness self is low, it is because it is associated to features that carry a low worthiness value. If the worthiness of the object is high, it is because it is associated to features that have a high worthiness value (Fig.~\ref{features}). In other words, the landscape of associated features constitutes the foundation of the traumatic structure. If the worthiness of such features is changed, we can expect the worthiness of the self and the object to change accordingly.

\subsection{Eating disorders}

\subsubsection*{Introduction}

\subsubsection*{Interpretation}

\clearpage

